The Second Fermi Large Area Telescope Catalog of Gamma-ray Pulsars

This catalog summarizes 117 high-confidence > 0.1 GeV gamma-ray pulsar detections using three years of data acquired by the Large Area Telescope (LAT) on the Fermi satellite. Half are neutron stars discovered using LAT data, through periodicity searches in gamma-ray and radio data around LAT unassociated source positions. The 117 pulsars are evenly divided into three groups: millisecond pulsars, young radio-loud pulsars, and young radio-quiet pulsars. We characterize the pulse profiles and energy spectra and derive luminosities when distance information exists. Spectral analysis of the off-peak phase intervals indicates probable pulsar wind nebula emission for four pulsars, and off-peak magnetospheric emission for several young and millisecond pulsars. We compare the gamma-ray properties with those in the radio, optical, and X-ray bands. We provide flux limits for pulsars with no observed gamma-ray emission, highlighting a small number of gamma-faint, radio-loud pulsars. The large, varied gamma-ray pulsar sample constrains emission models. Fermi's selection biases complement those of radio surveys, enhancing comparisons with predicted population distributions.

==> OffPeak/off_peak_auxiliary_description.tex <==
% \clearpage
\subsection{Description of Auxiliary information for Off-peak Analysis}
\label{off_peak_auxiliary}

A more complete list of the off-peak spectral and spatial 
results from the analysis described in Section~\ref{unpulsed}
is contained
in a supplemental FITS table.
\tabref{off_peak_aux} describes each of its columns.

For sources reported with a PL spectral model,
the differential spectrum is defined as
\begin{equation}\eqnlabel{powerlaw_definition}
  \dnde = \fitsformat{Prefactor} \left(\frac{E}{\fitsformat{Scale}}\right)^{-\fitsformat{Index}}
\end{equation}
\fitsformat{Prefactor}, \fitsformat{Index}, and \fitsformat{Scale} are specified in the table.
For sources reported with a PLEC1 spectral model (\fitsformat{\PLSuperExpCutoff}), the differential spectrum is defined as:
\begin{equation}\eqnlabel{cutoff_powerlaw_definition}
  \dnde = \fitsformat{Prefactor} \left(\frac{E}{\fitsformat{Scale}}\right)^{-\fitsformat{Index}} \exp\left(-\frac{E}{\fitsformat{Energy\_Cutoff}}\right)
\end{equation}
and \fitsformat{Prefactor}, \fitsformat{Index}, \fitsformat{Scale}, and \fitsformat{Energy\_Cutoff} are specified in the table.

For the Crab Nebula and Vela-X, we took the spectral shape and
initial normalization from \citet{LAT_collaboration_crab_2012} and
\cite{FermiVelaX2nd} respectively
and fit only a
multiplicative offset (see Section~\ref{off_peak_analysis}). For these two
sources, the differential spectrum was defined as
\begin{equation}\eqnlabel{filefunction_definition}
  \dnde = \fitsformat{Normalization} \left.\frac{dN}{dE}\right|_\mathrm{file}
\end{equation}
and the \fitsformat{Normalization} is defined in the auxiliary table.

% \clearpage
\begin{deluxetable}{p{1in} p{1in} p{3.5in}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Description of the Columns in the Off-Peak Auxiliary Fits Table
\tablabel{off_peak_aux}
}
\tablewidth{6in}
\input{OffPeak/tables/off_peak_auxiliary_table_description.tex}
\end{deluxetable}
\clearpage


==> OffPeak/tables/off_peak_auxiliary_table_description.tex <==
\tablehead{\colhead{Name} & \colhead{Units} & \colhead{Description}}
\startdata
\fitsformat{PSR}                           &                 & The name of the pulsar for which the off-peak region is studied. \\[\auxtablesep]
\fitsformat{Classification}                &                 & Off-peak emission class: \fitsformat{M} for magnetospheric (``pulsar-like''), 
%                                                               \fitsformat{M*} likely magnetospheric but with spatial analysis difficulties,
                                                               \fitsformat{W} for Pulsar Wind-like, and \fitsformat{U} for Unidentified.
                                                               \fitsformat{L} is for sources with no significant off-peak emission.\\[\auxtablesep]
\fitsformat{Off\_Peak\_Min}, 
\fitsformat{Off\_Peak\_Max}                &                 & The minimum and maximum phase that defines the off-peak interval. \\[\auxtablesep]
\fitsformat{Second\_Off\_Peak\_Min},                          
\fitsformat{Second\_Off\_Peak\_Max}        &                 & For pulsars with two off-peak phase ranges, the 
                                                               minimum and maximum phase for the second off-peak interval. \\[\auxtablesep]
\fitsformat{TS\_point}                     &                 & The test statistic obtained at the best-fit position of 
                                                               the assumed point-like source.
                                                               $\tspoint$ is computed at the best-fit position assuming a power-law spectral model (except for PSR\,J0534+2200
                                                               as is described in Section \ref{off_peak_analysis}). \\[\auxtablesep]
\fitsformat{TS\_ext}                       &                 & The significance of any possible extension 
                                                               for the source. \\[\auxtablesep]
\fitsformat{TS\_cutoff}                    &                 & The significance of any spectral cutoff for a source detected in the off-peak
                                                              region.
                                                              It is computed at the pulsar's position. \\[\auxtablesep]
\fitsformat{TS\_altdiff}                   &                 & The minimum significance of the source using the alternative diffuse models.
                                                               This is only computed for `M'-type and `M*'-type sources. \\[\auxtablesep]
\fitsformat{TS\_var}                    &                    & The significance of variability. \\[\auxtablesep]
\fitsformat{Spectral\_Model}               &                 & For regions with a significant detection, this is the best spectral model selected by 
                                                               our analysis procedure described in Section \ref{off_peak_analysis}.  The possible
                                                               spectral models are \fitsformat{PowerLaw}, \fitsformat{\PLSuperExpCutoff}, 
                                                               and \fitsformat{FileFunction} and are consistent with
                                                               naming convention in \gtlike. \\[\auxtablesep]
\fitsformat{Flux},
\fitsformat{Flux\_Error}                   & \fluxunits      & The best-fit photon flux and estimated statistical error. 
                                                               The flux is integrated from 100 \mev to 316 \gev. \\[\auxtablesep]
\fitsformat{EFlux},
\fitsformat{EFlux\_Error}                  & \efluxunits     & The best-fit energy flux and estimated statistical error. 
                                                               The flux is integrated from 100 \mev to 316 \gev. \\[\auxtablesep]
\fitsformat{Prefactor},
\fitsformat{Prefactor\_Error}              & \prefunits      & The best-fit prefactor and estimated statistical error 
                                                               for the \fitsformat{PowerLaw} and \fitsformat{\PLSuperExpCutoff} spectral models.
                                                               The prefactor is defined in \eqnref{powerlaw_definition} and 
                                                               \eqnref{cutoff_powerlaw_definition} for the two spectral models. \\[\auxtablesep]
\fitsformat{Normalization},
\fitsformat{Normalization\_Error}          &                 & The best-fit normalization and estimated statistical error for \fitsformat{FileFunction} spectral models. 
                                                               The normalization is defined in \eqnref{filefunction_definition}. This spectral model was only
                                                               used for the Crab Nebula and Vela$-$X. \\[\auxtablesep]
\fitsformat{Scale}                         & \mev            & The scaling energy for the \fitsformat{PowerLaw} and \fitsformat{\PLSuperExpCutoff} spectral models.
                                                               The scale is defined in \eqnref{powerlaw_definition} and 
                                                               \eqnref{cutoff_powerlaw_definition} for the two spectral 
                                                               models. \\[\auxtablesep]
\fitsformat{Index},
\fitsformat{Index\_Error}                  &                 & The best-fit spectral index and estimated statistical error 
                                                               for the \fitsformat{PowerLaw} and \fitsformat{PLSuperExpCutoff} spectral models.
                                                               The spectral index is defined in \eqnref{powerlaw_definition} and 
                                                               \eqnref{cutoff_powerlaw_definition} for the two 
                                                               spectral models. \\[\auxtablesep]
\fitsformat{Energy\_Cutoff},
\fitsformat{Energy\_Cutoff\_Error}         & \mev            & The best-fit cutoff energy and the estimated statistical error
                                                               for the \fitsformat{\PLSuperExpCutoff} spectral model. 
                                                               It is defined in \eqnref{cutoff_powerlaw_definition}. \\[\auxtablesep]
\fitsformat{Spatial\_Model}                &                 & For off-peak regions with a significant detection, the spatial model selected by
                                                               our analysis procedure described in Section \ref{off_peak_analysis}.
                                                               The choices are \fitsformat{At\_Pulsar}, \fitsformat{Point}, and \fitsformat{Extended}. \\[\auxtablesep]
\tablebreak
\fitsformat{RA\_J2000},
\fitsformat{DEC\_J2000}                    & deg          & The position of the source in celestial coordinates. 
                                                               For upper limits and sources with a best fit spatial 
                                                               model at the pulsar position, this is the pulsar's position.
                                                               For sources where the localized position is the selected
                                                               spatial model, this is the best-fit position.
                                                               For spatially-extended sources, this is the center
                                                               of the best-fit extended source spatial model. \\[\auxtablesep]
\fitsformat{GLON},
\fitsformat{GLAT}                          & deg          & This is the same as \fitsformat{RA\_J2000} and
                                                               \fitsformat{DEC\_J2000}, but in Galactic coordinates. \\[\auxtablesep]
\fitsformat{Position\_Error}               & deg          & For sources with a \fitsformat{Point} spatial model,
                                                               the estimated statistical error on the localization of the source. For sources
                                                               with an \fitsformat{Extended} spatial model, the 
                                                               estimated statistical error on the center of the extended source. \\[\auxtablesep]
\fitsformat{Extension},
\fitsformat{Extension\_Error}              & deg          & For sources with an \fitsformat{Extended} spatial model, the best fit extension
                                                               and estimated statistical error. \\[\auxtablesep]
\fitsformat{PowerLaw\_Flux\_UL}            & \fluxunits      & For regions with no significant detection, this is the 95\% confidence-level photon flux upper limit
                                                               computed assuming a power-law spectral model with $\fitsformat{Index}=2$
                                                               and integrated from 100 \mev to 316 \gev. \\[\auxtablesep]
\fitsformat{PowerLaw\_EFlux\_UL}           & \efluxunits     & The same as \fitsformat{PowerLaw\_Flux\_UL}, but instead the energy flux
                                                               integrated from 100 \mev to 316 \gev. \\[\auxtablesep]
\fitsformat{Cutoff\_Flux\_UL}              & \fluxunits      & For regions with no significant detection, the 95\% confidence-level photon flux upper limit
                                                               assuming an exponentially cutoff power-law spectral model with a canonical pulsar
                                                               spectrum of $\fitsformat{Index}=1.7$ and $\fitsformat{Energy\_Cutoff}=3$.
                                                               This is the flux upper limit integrated from 100 \mev to 316 \gev. \\[\auxtablesep]
\fitsformat{Cutoff\_EFlux\_UL}             & \efluxunits     & The same as \fitsformat{Cutoff\_Flux\_UL}, but instead the energy flux. \\[\auxtablesep]
\fitsformat{SED\_Lower\_Energy},                             
\fitsformat{SED\_Upper\_Energy},
\fitsformat{SED\_Middle\_Energy},          & \mev            & For each region, we computed a Spectral Energy Distribution (SED)
                                                               for the source in 14 energy bins spaced uniformly from 100 \mev 
                                                               to 316 \gev (4 bins per energy decade). Therefore, each 
                                                               \fitsformat{SED\_*} column corresponds to a vector of 14 values,
                                                               one for each energy bin.
                                                               \fitsformat{SED\_Lower\_Energy}, \fitsformat{SED\_Upper\_Energy}, and
                                                               \fitsformat{SED\_Middle\_Energy} are the lower energy, upper energy,
                                                               and energy in the geometric mean of the energy bin for each SED point. \\[\auxtablesep]
\fitsformat{SED\_TS}                       &                 & The test statistic obtained for each SED point. \\[\auxtablesep]
\fitsformat{SED\_Prefactor},
\fitsformat{SED\_Prefactor\_Lower\_Error},
\fitsformat{SED\_Prefactor\_Upper\_Error},
\fitsformat{SED\_Prefactor\_UL}            & \prefunits      & The best-fit prefactor, asymmetric lower and upper error, and
                                                               95\% confidence-level upper limit computed
                                                               for the source in each energy bin.
                                                               When $\tspoint\geq25$, a detection is quoted 
                                                               when $\fitsformat{SED\_TS}>4$
                                                               and an upper limit is quoted otherwise. When $\tspoint<25$,
                                                               all SED points are quoted as upper limits. \\[\auxtablesep]
\enddata

